Vague Preference Policy Learning for Conversational Recommendation

Conversational recommendation systems (CRS) commonly assume users have clear preferences, leading to potential over-filtering of relevant alternatives. However, users often exhibit vague, non-binary preferences. We introduce the Vague Preference Multi-round Conversational Recommendation (VPMCR) scenario, employing a soft estimation mechanism to accommodate users' vague and dynamic preferences while mitigating over-filtering. In VPMCR, we propose Vague Preference Policy Learning (VPPL), consisting of Ambiguity-aware Soft Estimation (ASE) and Dynamism-aware Policy Learning (DPL). ASE captures preference vagueness by estimating scores for clicked and non-clicked options, using a choice-based approach and time-aware preference decay. DPL leverages ASE's preference distribution to guide the conversation and adapt to preference changes for recommendations or attribute queries. Extensive experiments demonstrate VPPL's effectiveness within VPMCR, outperforming existing methods and setting a new benchmark. Our work advances CRS by accommodating users' inherent ambiguity and relative decision-making processes, improving real-world applicability.

==> sections/4.framework.tex <==

\begin{figure*}[t]
    \centering
	\includegraphics[width=\linewidth]{figs/method.pdf}
	%\vspace{-5pt}
    \caption{Overview of the proposed method for the vague preference multi-round conversational recommendation.}
    \label{fig:method-exa}
\end{figure*}

\section{FRAMEWORK}
\label{sec:method}

we propose \emph{Choice-based Vague Preference Policy Learning} (CVPPL), a general solution framework for VPMCR. The whole conversation process is decomposed into three steps: \textit{tracking}, \textit{consultation}, and \textit{transition}.  

\subsection{Tracking}
\label{sec:framework_tracking}
In the tracking stage, user preference modeling and conversation state representation should be dynamically modeled based on the feedback of the user's choice in each round. This stage is triggered when the user initializes the conversation by specifying a fine-grained attribute or when the user makes a choice about fine-grained attributes asked by CRS.
\subsubsection{User Preference Modeling} 
\label{sec:framework_tracking_user}
In a choice-based interaction setting ~\cite{zhang2022multiple}, the user needs to make selections from a tiny set of attributes or items in each round. 

Given the ambiguity and imprecision of user behavior, we employ a soft analysis approach to analyze user click behavior. Drawing from the diversity of the choice set, we consider both explicit and implicit information conveyed by the user behavior set ($\mathcal{P}_{click}^t$ or $\mathcal{P}_{n\mbox{-}click}^t$)  and the system undisplayed set ($\mathcal{P}_{n\mbox{-}ask}^t$) with respect to item $v$. Based on the psychology of user decision-making, we estimate the importance and potential importance of both the user-clicked choices and the user-unclicked choices for item $v$. 
\begin{equation}
\label{eq:w_v_click}
    w_{v\mbox{-}click}^t=\text{Information}(v, \mathcal{P}_{click}^t, \mathcal{P}_{n\mbox{-}ask}^t), 
\end{equation}
\begin{equation}
\label{eq:w_v_not_click}
    w_{v\mbox{-}nclick}^t=\text{Information}(v, \mathcal{P}_{n\mbox{-}click}^t, \mathcal{P}_{n\mbox{-}ask}^t), 
\end{equation}
where $w_{v\mbox{-}click}^t$ and $w_{v\mbox{-}nclick}^t$ represents the user choice-based information score.

The previous dynamic user preference modeling methods ~\cite{lei20estimation, lei2020interactive, xu2021adapting, deng2021unified, zhang2022multiple} consider modeling all the feedback signals in the user's conversation history together. However, this mixed signal will induce noise and cannot capture the user's vague and changeable preferences well. Therefore, modeling the user's choice behavior at each round separately is considered a more reliable analysis mode for inferring the current user's intention. That is, in each round of interaction, user preference modeling can be divided into personalized user modeling and click behavior modeling. Personalized user modeling considers the static preference of users for items, and click behavior modeling considers the user's click signal and non-click signal, in which the user's current choice intention to the item $v$ is affected by the shared information transmission of click attributes $\mathcal{P}_{click}^t$ and non-click attributes $ \mathcal{P}_{n\mbox{-}click}^t$ in current round $t$. 
\begin{equation}
\label{eq:w_v_current}
    w_v^t=\sigma (w_{v\mbox{-}u}^t + w_{v\mbox{-}click}^t + w_{v\mbox{-}nclick}^t), 
\end{equation}

% \vspace{-5pt}
% \begin{equation}
% \label{eq:w_p}
%     w_p^t=Information(u, p, \mathcal{P}_{click}^t, \mathcal{P}_{n\mbox{-}click}^t), 
% \end{equation}
where $w_v^t$ is a scalar score indicating the user's current confidence towards the item $v$ in current round $t$ and $w_{v\mbox{-}u}^t$ represents the user personalized information score. $\sigma$ denotes the sigmoid function. 

As the number of interactions increases, CRS endeavors to elicit the user's preferences, and the user's personal intention space evolves from being ambiguous to become clearer. Furthermore, there may be fluctuations in the user's interests and preferences. Thus, the actual intention space of the user should be viewed as a coalescence of the user intention from all interactions. As a result, the user's actual perception of the item should be reflected as: 
\begin{equation}
\label{eq:w_v_real}
    w_v=\text{Combination}(\alpha_{1} w_v^1, \alpha_{2}w_v^2, ..., \alpha_{t}w_v^t), 
\end{equation}
where $w_v$ is a scalar score indicating the inferred user's real confidence towards the item $v$ from the first round to the current round $t$ and $\{ \alpha_{1}, \alpha_{2}, ... \alpha_{t} \}$ are the weight coefficients.   

Moreover, the user‘s preference distribution over the candidate items $f_u^t(v)$ is easy to derive by calculating the user's real confidence for all items in the candidate item set $\mathcal{V}_{cand}^t$. 
\begin{equation}
\label{eq:W_v_cand}
    f_u^t(v)= \{ w_{v_1}, w_{v_2}, ..., w_{v_{n}} \}. 
\end{equation}
where $n$ denotes the number of candidate items in round $t$.

Naturally, utilizing the user's genuine belief $w_p$ about attribute $p$, the user‘s preference distribution over the candidate attributes $f_u^t(p)$ can be also represented similarly.

\subsubsection{Conversation State Representation} 
\label{sec:framework_tracking_conversation}

The user's historical state throughout the session should also be captured. For this reason, the history session state  $s_{his}^t$ containing the user's historical behavior trajectory should also be represented. As a result, each round of the user's historical click attributes $\mathcal{P}_{click}$ are recorded by the history session state $s_{his}^t$ throughout the session.
\begin{equation}
\label{eq:s_his}
    s_{his}^t= \mathcal{P}_{click} = \{\mathcal{P}_{click}^1, \mathcal{P}_{click}^2, ...,  \mathcal{P}_{click}^t\}, 
\end{equation}


In addition to the historical conversation state, a dynamic conversation state is needed to represent the changing conversation interaction in each round. So a flexible conversation state should be designed to discover the changing interrelationships among different items and attributes in the current interaction round. Thus, the current conversation state $s_{cur}^t$ should includes user $u$, user's historical click attributes $\mathcal{P}_{click}$, the candidate items $\mathcal{V}_{cand}^t$ and the candidate attributes $\mathcal{P}_{cand}^t$ in current round $t$.
\begin{equation}
\label{eq:s_cur}
    s_{cur}^t= \{u, \mathcal{P}_{click}, \mathcal{V}_{cand}^t, \mathcal{P}_{cand}^t\}, 
\end{equation}

Finally, the conversation state representation $\mathcal{S}_{conv}^t$ is encoded by the current conversation state and historical session states: 
\begin{equation}
\label{eq:s_conv}
    \mathcal{S}_{conv}^t= Encoder(s_{cur}^t, s_{his}^t).
\end{equation}


\subsection{Consultation}
\label{sec:framework_consultation}
In the consultation stage, a unified policy learning that incorporates user preference modeling information and conversation state representation information conducts the reasonable CRS decision about what items to recommend or what attributes to ask. Specifically, at each round $t$, a policy function $\pi(\mathbf{s})$ is expected to make the decision $\mathcal{A}_{CRS}^t$ (i.e., asking certain attribute $\mathcal{A}_{ask}^t$  or recommended certain items $\mathcal{A}_{rec}^t$ ) that maximizes the gain of the whole  session in the context of user preference distribution over items $W_{\mathcal{V}_{cand}}^t$, user preference distribution over attributes $W_{\mathcal{P}_{cand}}^t$ and conversation state $\mathcal{S}_{conv}^t$. 

\begin{equation}
\label{eq:a_policy}
    \mathcal{A}_{CRS}^t = \pi(\mathbf{s}) = \pi(W_{\mathcal{V}_{cand}}^t, W_{\mathcal{P}_{cand}}^t, \mathcal{S}_{conv}^t).
\end{equation}

It is worth mentioning that the policy action space $\mathcal{A}^t$ usually involves all candidate items  $\mathcal{V}_{cand}^t$ and all candidate attributes $\mathcal{P}_{cand}^t$ at each round $t$. When the action space becomes overwhelmingly large, it requires a tremendous amount of interaction data to optimize the policy, and sparse interaction data also means that the difficulty of policy training increases sharply ~\cite{deng2021unified}.  In conclusion, an effective action-pruning strategy is needed to improve the sampling efficiency and reduce the computational complexity of the model. This strategy is expected to select the action space that is most beneficial to the long-term gain of the CRS.
\begin{equation}
\label{eq:a_sub}
\begin{split}
    \mathcal{A}_{sub}^t = \text{Selection}(\mathcal{V}_{cand}^t,\mathcal{P}_{cand}^t). 
\end{split}
\end{equation}

where $\mathcal{A}_{sub}^t$ means a small subset of actions selected from the entire action space $\mathcal{A}^t$ using the pruning strategy in the current round $t$. Thus, the policy function only makes decision $\mathcal{A}_{CRS}^t$ from a small subspace of the whole action space, which denotes as $\mathcal{A}_{CRS}^t \subset  \mathcal{A}_{sub}^t $.

\subsection{Transition}
\label{sec:framework_transition}
Finally, the transition stage well triggered after the consultation stage is finished. In this stage, the candidate item set $\mathcal{V}_{cand}^t$ and the candidate attribute set $\mathcal{P}_{cand}^t$ are updated by CRS. In the VPMCR setting, instead of using strong feedback signals from the user as indicators to filter items, each item is considered to have the potential to be liked by the user (i.e., CRS will infer that any item might be a member of the target item set $\mathcal{V}_{target})$. Therefore, $\mathcal{V}_{cand}^t$ will update only when CRS conducts recommended actions $\mathcal{A}_{rec}^t$ (i.e., show the recommended list $\mathcal{V}_{rec}^t$). This update process is represented as: 
\begin{equation}
\label{eq:update_vcand}
    \begin{array}{l}
    \mathcal{V}_{cand}^t=
    \left\{\begin{array}{ll}
        \mathcal{V}_{cand}^t \setminus {\mathcal{V}_{rec}^t}, & \text { if }  \quad {\mathcal{V}_{target}} \cap {\mathcal{V}_{rec}^t} = \emptyset \\
        \mathcal{V}_{cand}^t \cap {\mathcal{V}_{rec}^t}, & \text { if } \quad {\mathcal{V}_{target}} \cap {\mathcal{V}_{rec}^t} \neq \emptyset 
    \end{array}\right.
    \end{array}
\end{equation}

Similarly, after CRS conducts asking actions $\mathcal{A}_{ask}^t$ (i.e.,  the displayed attributes $\mathcal{P}_{ask}^t$), the candidate attribute set $\mathcal{P}_{cand}^t$ update process is represented as:
\begin{equation}
\label{eq:update_pcand}
    \mathcal{P}_{cand}^t = \mathcal{P}_{cand}^t \setminus \mathcal{P}_{ask}^t.
\end{equation}

Instead of updating the candidate item set fixedly, the candidate attributes set is allowed to use additional attribute pruning strategies ~\cite{lei2020interactive} to reduce the space of candidate attribute set $\mathcal{P}_{cand}^t$ in each round $t$.
